A Semi-supervised Graph Attentive Network for Financial Fraud Detection

With the rapid growth of financial services, fraud detection has been a very important problem to guarantee a healthy environment for both users and providers. Conventional solutions for fraud detection mainly use some rule-based methods or distract some features manually to perform prediction. However, in financial services, users have rich interactions and they themselves always show multifaceted information. These data form a large multiview network, which is not fully exploited by conventional methods. Additionally, among the network, only very few of the users are labelled, which also poses a great challenge for only utilizing labeled data to achieve a satisfied performance on fraud detection. To address the problem, we expand the labeled data through their social relations to get the unlabeled data and propose a semi-supervised attentive graph neural network, namedSemiGNN to utilize the multi-view labeled and unlabeled data for fraud detection. Moreover, we propose a hierarchical attention mechanism to better correlate different neighbors and different views. Simultaneously, the attention mechanism can make the model interpretable and tell what are the important factors for the fraud and why the users are predicted as fraud. Experimentally, we conduct the prediction task on the users of Alipay, one of the largest third-party online and offline cashless payment platform serving more than 4 hundreds of million users in China. By utilizing the social relations and the user attributes, our method can achieve a better accuracy compared with the state-of-the-art methods on two tasks. Moreover, the interpretable results also give interesting intuitions regarding the tasks.

==> model.tex <==
\section{The Model}

\subsection{Data Descriptions and Notations}
\begin{figure}[htb]
\centering
\includegraphics[width=0.4\textwidth]{pics/framework.pdf}
\caption{The data illustrations. Some users are labeled and most users are unlabeled. We have the most users' nicks and their frequently-used addresses.}
\label{pic:data_framework}
\end{figure}

We first give a brief description of our data for the problem, which can be shown in Figure \ref{pic:data_framework}. Generally, we use three views of data: social relations, address data and nicks data. The assumption of using social relations is that people of similar occupations will form a dense cluster. The address can directly indicate the work and home address, which can directly reflect the people's job. The nick data is generated online by other people. The assumption of using nicks is that how people describe a person, which we call nicks like Doctor Jack, may also show his occupation. 

In detail, we first build the user-relation graph $G^{(U)}=\{U, E^{(U)}\}$. The users $U$ is composed of $U_l$ and $U_{ul}$, where $U_l$ denotes the users with known occupations and $U_{ul}$ denotes the users without known occupations. $|U_{ul}| >> |U_l|$. $E^{(U)}$ denotes the relationships between users. Here, in our problem if two users are labeled as friends, classmates or workmates, there will be an undirected edge with weight $1$ for simplicity between the two users. 

Besides, users usually upload their frequently-used addresses for online merchant. One address is usually a sentence containing the country, province (state), city, street and door information of the user. For most of the users, they have at least one address. We perform word-cut algorithm to seperate each address into several address-related words. If the user's address contains a word, we set a link between the user and the word. In this way, each user will link to several words, which forms a user-word bipartite graph $G^{(UA)}=\{U \cup S^{(A)}, E^{(UA)}\}$, where $S^{(A)}$ denotes word vocabulary regarding the addresses and $E^{(UA)}$ denotes the edges between the users and the address-related words. The edge's weight is corresponding to the word frequency.  

Finally, we utilize the user's nicks. We use $n_{1,2}$ to denote the nicks user $u_1$ marks to user $u_2$. Similarily, we can seperate each nick into the words. Then for each user $u$, we will assemble all the words from $\bigcup_{v \in U} n_{vu}$ as the user $u$'s nick-related words. In this way, we can build user-nick bipartite graph $G^{(UN)}=\{U \cup S^{(N)}, E^{(UN)}\}$, where $S^{(N)}$ denotes word vocabulary regarding the nicks and $E^{(UN)}$ denotes the edges between the users and the nick-word. 

\subsection{\methodshort}
\begin{figure*}[htb]
\centering
\includegraphics[width=0.75\textwidth]{pics/model.pdf}
\caption{The framework of the proposed model \methodshort. }
\label{pic:model_framework}
\end{figure*}

\subsubsection{Overall Architectures}
In this section, we introduce how our proposed model \methodshort{} utilizes multiview data: $G^{(U)}$, $G^{(UA)}$ and $G^{(UN)}$ for occupation prediction. The framework of the whole model can be shown in Figure \ref{pic:model_framework}. For multiview data, due to their different statistical properites existing in raw data, we first use seperate models to project multiview data into the high-level space and then integrate them to obtain the high-level joint embeddings. With the joint embeddings, we design the supervised classification loss and unsupervised graph-based loss to fully utilize the labeled and unlabeled data. 

In detail, in $G^{(UA)}$, for a user $u$, we denote its neighbors, i.e. address-related words as $S_u^{(A)}=\{s_{u1},...,s_{un}\}$ with the weights $\{w_{u1},...,w_{un}\}$, where each $s_{ui}$ denotes a word and $w_{ui}$ denotes its frequency. Let $W^{(A)}\in R^{|V^{A}|\cdot d}$ denote the embedding matrix of address-related vocabulary, where $|V^{A}|$ denotes the vocabulary size and $d$ denotes the dimension size. We use $W^{(A)}(a)$ to denote the embedding look-up operation for the word $a$. Then the weighted word embedding of word $s_{ui}$ can be calculated as $w_{ui} \cdot W^{(A)}(s_{ui})$, which we simply denote as $e_{ui}$. Then we hope to aggregate the embedding of the word to obtain the address-related user embeddings. However, different words contribute unequally to the final occupations. Therefore, we propose a word-attention mechanism. In detail, let $H \in R^{|V^{A}|\cdot d}$ be a learnable parameter. Then the importance $\alpha_{ui}$ of the word $s_{ui}$ can be defined as follows:
\begin{equation}
\alpha_{ui} = \frac{exp(e_{ui}\cdot H_{ui,\cdot})}{\sum_{s \in S_u^{(A)}}{exp(e_s\cdot H_{s\cdot})}}. \nonumber
\end{equation}

Once obtained $\alpha_{ui}$, in the words assembling layer of Figure \ref{pic:model_framework}, the normalized importance is used to compute a linear combination of the word embeddings to obtain the address-related user embeddings:
\begin{equation}
h_{u}^{(A)} = \sum_{s \in S_u^{(A)}}{\alpha_{s}e_{s}}. \nonumber
\end{equation}

Similarily, we can obtain the nick-related user embeddings $h_{u}^{(N)}$ also by using word-attention mechanism. However, the nick-related user embeddings $h_{u}^{(N)}$ and the address-related embeddings $h_{u}^{(A)}$ lie in heterogeneous domains. They have different statistical properties, which makes them difficult to capture the multiview correlations in this space. To address the problem, we use separate multi-layer perceptrons (MLP), shown as view-specific layer in Figure \ref{pic:model_framework}, to project multiview data into the high-level space first.  The representations of the $l$-layer are defined as: 
\begin{equation}
h_{u}^{(X)_l} = Relu(h_{u}^{(X)_{l-1}}W_l^{(X)}), X\in\{A,N\} ,  \nonumber
\end{equation}
where $h_{u}^{(X)_0}=h_{u}^{(X)}$.

Through several layers of non-linear functions to map the raw data into the high-level space, it is easier to correlate multiview data \cite{b30}. Considering that different views contribute differently, we propose a view-attention mechnism for multiview data. Specifically, we use $\phi^A$ and $\phi^N$ to denote learnable parameters for address view and nick view. Then the importance of each view is: 
\begin{equation}
\alpha_{X} = \frac{exp(h_{u}^{(X)_L} \cdot \phi^X)}{\sum\limits_{D \in \{A,N\}}{exp(h_{u}^{(D)_{L}}\cdot \phi^D)}},X\in\{A,N\}, \nonumber
\end{equation}
where $L$ is the number of layers for the seperate models. 

Then we can obtain the view-integrated features:
\begin{equation}
h_{u} = \alpha_{A} h_{u}^{(A)_{L}}\ ||\ \alpha_{N} h_{u}^{(N)_{L}},  \nonumber
\end{equation}
where $||$ denotes the concatenation operation.

Finally, we use a one-layer perceptron, which uses the integrated features $h_{u}$ as the input to refine the representations. After that,  we can obtain the final high-level embeddings for the user $u$ in the embedding layer, which we denote as $a_{u}$. With $a_{u}$ for each user, we can define the task-specific loss functions, which we leave in the next section. 

\subsubsection{Loss function and Optimization}
For the users with labels, we use a softmax on the representations of the embedding layer to get the classification result. Thus we can define the classification loss: 
\begin{equation}
\mathcal{L}_{sup} = -\frac{1}{|U_L|}\sum\limits_{u\in U_l}\sum\limits_{i=1}^k{1{(y_u=i)}}\ log\frac{exp(a_u\cdot \theta_i)}{\sum\limits_{j=1}^k{exp(a_u\cdot \theta_j)}},
\label{eqn:sup}
\end{equation}
where $I(\cdot)$ is the indicator function and $k$ is the number of occupations to be predicted.

However, very few users will upload their occupations online, which makes the model difficult to learn a good classifier with such limited labeled data. Although for a huge number of users we do not have their occupations, we have their addresses and the nicks. Furthermore, we know their social relations to the users with known occupations. In this way, we can utilize the social relations to bridge the labeled and unlabeled data and thus learn the model with the unlabeled data. To achieve this, inspired by Deepwalk \cite{b19}, we propose an unsupervised graph-based loss function to refine the whole model. Given the relation graph $G^{(U)}$, we perform random walk to define the neighbors of each vertex. The loss function encourages nearby nodes having similar representaions while makes the representations of disparate nodes distinct:
\begin{eqnarray}
\mathcal{L}_{graph}=\sum\limits_{u \in U}\sum\limits_{v\in N_u \cup Neg_u}-log(\sigma(a_u^Ta_v)) \nonumber\\ 
-Q\cdot E_{q \sim P_{neg}(u)}log(\sigma(a_u^Ta_q)), 
\label{eqn:unsup}
\end{eqnarray}
where $v$ is a node that co-occurs in the $u$'s random walk path, $\sigma$ is the sigmoid function, $P_{neg}(u) \propto d_u^{0.75}$ is the negative sampling distribution and $Q$ is the number of negative samples set to $3$ in our paper. 

More importantly, the embedding $a_u$ we feed into the loss function is generated from the user's textual contents, rather than directly performing embedding look-up. In this way, we not only utilize the social relations of the unlabeled data, but also integrate their content information, which further improves the model's performance. 

Then we combine the supervised classification loss (Eqn. \ref{eqn:sup}) and unsupervised graph loss (Eqn. \ref{eqn:unsup}) to form the final objective function: 
\begin{equation}
\mathcal{L}_{\methodshort{}}=\mathcal{L}_{sup}+\mathcal{L}_{graph}
\label{eqn:loss}
\end{equation}

We optimize the model using Stochastic Gradient Descent (SGD). The pseudo code to train \methodshort{} is listed in Alg. \ref{alg:train}.
\begin{algorithm}[htb]
\caption{Training Algorithm for \methodshort{}}
\label{alg:train}
\begin{algorithmic}[1]
\REQUIRE $G^{(U)}$, $G^{(UA)}$, $G^{(UN)}$
\ENSURE The model parameters
\STATE Initializing all the parameters of the model $\Theta$. 
\STATE Generating random walk paths according to $G^{(U)}$ and construct the user paired set S.
\FORALL{$(u,v) \in S$}
\STATE Obtain $a_u$ and $a_v$ according to the model architecture. 
\STATE Get $\mathcal{L}_{\methodshort{}}$ according to Eqn. \ref{eqn:loss}.
\STATE $\Theta^{(new)}=\Theta^{(old)}-\lambda \cdot \frac{\partial{\mathcal{L}_{\methodshort{}}}}{\partial{\Theta^{(old)}}}$
\ENDFOR
\end{algorithmic}
\end{algorithm}








